Ranking Regularization for Critical Rare Classes: Minimizing False Positives at a High True Positive Rate

In many real-world settings, the critical class is rare and a missed detection carries a disproportionately high cost. For example, tumors are rare and a false negative diagnosis could have severe consequences on treatment outcomes; fraudulent banking transactions are rare and an undetected occurrence could result in significant losses or legal penalties. In such contexts, systems are often operated at a high true positive rate, which may require tolerating high false positives. In this paper, we present a novel approach to address the challenge of minimizing false positives for systems that need to operate at a high true positive rate. We propose a ranking-based regularization (RankReg) approach that is easy to implement, and show empirically that it not only effectively reduces false positives, but also complements conventional imbalanced learning losses. With this novel technique in hand, we conduct a series of experiments on three broadly explored datasets (CIFAR-10&100 and Melanoma) and show that our approach lifts the previous state-of-the-art performance by notable margins.

==> chapters/supp_intro.tex <==
In this document, we provide details of missing components, like datasets, 

==> figures/abl_dequeue.tex <==
% \begin{table}
% \begin{tabular}{l | a | b | a | b}
% \hline
% \rowcolor{Goldenrod}
% \mc{1}{$\beta$}  & \mc{1}{98} & \mc{1}{95} & \mc{1}{92} & \mc{1}{AUC} \\
% \hline
% S 1 & a & b & c & d \\
% variable 2 & a & b & c & d \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[t]
% \centering % Centres the table on the page, comment out to left-justify
% \resizebox{0.5\columnwidth}{!}{%
% \begin{tabular}{l c c c c c} 
% % \begin{tabular}{l | a | b | a | b}
% \toprule
% % \rowcolor{Goldenrod}
% FPR@$\beta$TPR  & \mc{1}{98} & \mc{1}{95} & \mc{1}{92} & \mc{1}{AUC} \\
% \midrule
% Dequeue Max & c & b & c & d \\
% Dequeue Min & a & b & c & d \\
% FIFO & a & b & c & d \\
% \bottomrule
% \end{tabular}
% }
% \caption{ Comparing queuing strategy for the buffer.
% } 
% \label{tab:dequeue} 
% \end{table}

% \begin{table}[t]
% \setlength{\tabcolsep}{2.5pt}
% \caption{\textbf{Ablation study on batch sampling.} ``With sampling" refers to sampling $\mathcal{M}$ from the current batch such that each label occurs at most once. Results are on \textit{IMDB-WIKI-DIR} and \textit{AgeDB-DIR} with SQINV re-weighting, and \textit{STS-B-DIR} with Vanilla. We apply sampling in all other experiments.}
% \vspace{-4pt}
% \label{table:abltion_ties}
% \small
% \vskip 0.15in
% \begin{center}
% \resizebox{0.48\textwidth}{!}{
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllllcllll@{}}\toprule[1.2pt]
\multicolumn{1}{c}{\multirow{ 2}{*}{FPR@98TPR}} & \multicolumn{4}{c}{\textbf{Scaling factor $\lambda$ }} & \phantom{abc}& \multicolumn{4}{c}{\textbf{Smoothing factor} $\tau$} \\

\cmidrule{2-5} \cmidrule{7-10}
    & 1   & 2  & 4 & 8   &&  1   & 1.5   & 2 & 4\\
\midrule
BCE + RankReg
& 53.5 & 50.8 & 52.3 & 57.9 && 53.5 & 52.1 & 50.2 & 48.7 \\
A-FL + RankReg
& 49.6 & 53.6 & 50.3  & 53.3 && 49.6 & 48.6 & 50.8 & 47.5 \\
S-ML + RankReg
& 50.0 & 43.2 & 50.3 & 56.9 && 50.0 & 48.6 & 49.9 & 46.3 \\
CBBCE + RankReg
& 60.2 & 57.1 & 57.1  & 57.1 && 60.2 & 57.8 & 40.3 & 48.8 \\
%  \midrule
% Dequeue Max 
% & \textbf{6.91} & \textbf{6.34} & \textbf{7.79}   & \textbf{9.89} && \textbf{4.28} & \textbf{3.92} & \textbf{4.88} & {6.89} \\
% Dequeue Min 
% & 7.10 & 6.52 & 7.99 & 10.17 && 4.53 & 4.17 & 5.16 & \textbf{6.85} \\ 
% FIFO 
% & 7.10 & 6.52 & 7.99 & 10.17 && 4.53 & 4.17 & 5.16 & \textbf{6.85} \\
\bottomrule[1.2pt]
\end{tabular}
}
\caption{Ablation study on parameter sensitivity (top section).}
\end{table}

==> patent_tables.tex <==
\begin{table}[t]
\small
\centering % Centres the table on the page, comment out to left-justify
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l c c c c} 
\toprule % Top horizontal line
& \multicolumn{4}{c}{Binary CIFAR10, imb. \textbf{1:100}} \\
% \cmidrule[\RuleThicknessNormal](l{\RuleOffsetLeft})
\cmidrule(l){2-5} 
Methods & \vtop{\hbox{\strut FPR@ $\downarrow$}\hbox{\strut  98\%TPR}} & \vtop{\hbox{\strut FPR@ $\downarrow$}\hbox{\strut  95\%TPR}} &\vtop{\hbox{\strut FPR@ $\downarrow$}\hbox{\strut  92\%TPR}} &  AUC $\uparrow$ \\ % Column names row
\midrule % In-table horizontal line
BCE & 56.0 & 45.0 & 29.0 &  91.2 \\ % Content row 1
+ALM  & 52.0 & 34.0 & 21.0 & 93.1\\ % Content row 1
+RankReg   & \underline{\textbf{47.1}} & \underline{\textbf{26.2}} & \underline{\textbf{20.6}} & \textbf{\cl{red!60!white}{94.3}} \\ % Content row 1
\midrule
S-ML & 59.0 & 40.0 & 26.0 &  91.7 \\ % Content row 1
+ALM  & 50.0 & 37.0 & \underline{\textbf{24.0}} &  92.5\\ % Content row 1
+RankReg  & \underline{\textbf{45.6}} & \underline{\textbf{31.4}} & 29.7 &  \textbf{\cl{red!60!white}{93.9}} \\ % Content row 1
\midrule
S-FL & 59.0 & 40.0 & 27.0 &  91.7 \\ % Content row 1
+ALM  & 55.0 & 39.0 & 25.0 &  91.5\\ % Content row 1
+RankReg   & \underline{\textbf{53.3}} & \underline{\textbf{35.4}} & \underline{\textbf{20.7}}  & \textbf{\cl{red!60!white}{92.8}} \\ % Content row 1
\midrule
A-ML & 54.0 & 36.0 & 23.0 &  92.4 \\ % Content row 1
+ALM & \underline{\textbf{45.0}} & 35.0 & 23.0 &  92.8\\ % Content row 1
+RankReg  & 47.8 & \underline{\textbf{28.9}} & \underline{\textbf{21.4}} &  \textbf{\cl{red!60!white}{94.1}} \\ % Content row 1
\midrule
A-FL & 50.0 & 38.0 & 24.0 &  92.3 \\ % Content row 1
+ALM & \underline{\textbf{49.0}} & 37.0 & 23.0 &  92.8\\ % Content row 1
+RankReg  & 50.5 & \underline{\textbf{28.7}} & \underline{\textbf{20.9}} &  \textbf{\cl{red!60!white}{94.3}} \\ % Content row 1
\midrule
CB-BCE & 89.0 & 72.0 & 59.0 &  78.0 \\ % Content row 1
+ALM  & 67.0 & 51.0 & 36.0 &  88.1\\ % Content row 1
+RankReg   & \underline{\textbf{48.8}} & \underline{\textbf{29.9}} & \underline{\textbf{24.6}} & \textbf{\cl{red!60!white}{93.2}} \\ % Content row 1
\midrule
W-BCE & 69.0 & 52.0 & 37.0 &  87.4 \\ % Content row 1
+ALM  & 66.0 & 48.0 & 31.0 &  89.3\\ % Content row 1
+RankReg  & \underline{\textbf{60.0}} & \underline{\textbf{39.4}} & \underline{\textbf{29.6}} &  \textbf{\cl{red!60!white}{92.1}} \\ % Content row 1
\midrule
LDAM & 65.0 & 48.0 & 34.0 &  89.0 \\ % Content row 1
+ALM  & 60.0 & 42.0 & 31.0 &  91.0\\ % Content row 1
+RankReg  & \underline{\textbf{42.8}} & \underline{\textbf{25.6}} & \underline{\textbf{23.8}} &  \textbf{\cl{red!60!white}{95.0}} \\ % Content row 1
\midrule
\textcolor{Green}{Avg.} $\Delta$ & \textcolor{Green}{6.0}  & \textcolor{Green}{9.7} & \textcolor{Green}{2.8} & \textcolor{Green}{2.3} \\
\bottomrule % Bottom horizontal line

\end{tabular}
}
\caption{
Comparison results for binary imbalanced CIFAR-10. Baseline numbers are quoted from ALM~\cite{alm}.
} 
\label{tab:cifar10_imb100} 
\end{table}


\begin{table}[t]
\small
\centering % Centres the table on the page, comment out to left-justify
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l c c c c} 
\toprule % Top horizontal line
& \multicolumn{4}{c}{Binary CIFAR100, imb. \textbf{1:100}} \\ % 
\cmidrule(l){2-5} 
Methods & \vtop{\hbox{\strut FPR@ $\downarrow$}\hbox{\strut  98\%TPR}} & \vtop{\hbox{\strut FPR@ $\downarrow$}\hbox{\strut  95\%TPR}} &  \vtop{\hbox{\strut FPR@ $\downarrow$}\hbox{\strut  90\%TPR}} & AUC $\uparrow$ \\ % Column names row
\midrule % In-table horizontal line
BCE & 93.0 & 63.0 & 47.0 & 81.8 \\ % Content row 1
+ALM  & 91.0 & 49.0  & 39.0 & 82.7\\ % Content row 1
+RankReg   & \underline{\textbf{85.2}} & \underline{\textbf{42.4}}  & \underline{\textbf{28.7}} & \textbf{\cl{red!60!white}{85.5}} \\ % Content row 1
\midrule
S-ML & 89.0 & 65.0  & 43.0 & 82.7 \\ % Content row 1
+ALM  & 88.0 & 69.0  & 41.0 & 81.7\\ % Content row 1
+RankReg  & \underline{\textbf{64.0}} & \underline{\textbf{44.8}}  & \underline{\textbf{34.5}} & \textbf{\cl{red!60!white}{85.4}} \\ % Content row 1
\midrule
S-FL & 89.0 & 62.0  & 44.0 & 82.6 \\ % Content row 1
+ALM  & 88.0 & 60.0  & 42.0 & 81.7\\ % Content row 1
+RankReg   & \underline{\textbf{84.6}} & \underline{\textbf{49.2}} & \underline{\textbf{38.4}} & \textbf{\cl{red!60!white}{84.7}} \\ % Content row 1
\midrule
A-ML & 91.0 & 63.0  & 44.0 & 81.8 \\ % Content row 1
+ALM & 89.0 & 55.0  & 37.0 & 82.7\\ % Content row 1
+RankReg  & \underline{\textbf{81.6}} & \underline{\textbf{43.4}}  & \underline{\textbf{32.6}} & \textbf{\cl{red!60!white}{85.5}} \\ % Content row 1
\midrule
A-FL & 88.0 & 63.0  & 45.0 & 82.8 \\ % Content row 1
+ALM & 86.0 & 62.0  & 40.0 & 83.2\\ % Content row 1
+RankReg  & \underline{\textbf{70.0}} & \underline{\textbf{53.4}}  & \underline{\textbf{35.8}} & \textbf{\cl{red!60!white}{84.6}} \\ % Content row 1
\midrule
CB-BCE & 93.0 & 75.0  & 52.0 & 78.8 \\ % Content row 1
+ALM  & \underline{\textbf{89.0}} & 59.0  & 36.0 & 83.8 \\ % Content row 1
+RankReg   & 89.8 & \underline{\textbf{48.6}} & \underline{\textbf{33.4}} & \textbf{\cl{red!60!white}{84.1}} \\ % Content row 1
\midrule
W-BCE & 88.0 & 59.0  & 41.0 & 79.7 \\ % Content row 1
+ALM  & 87.0 & \underline{\textbf{53.0}}  & \underline{\textbf{39.0}} & \textbf{\cl{red!60!white}{83.2}} \\ % Content row 1
+RankReg  & \underline{\textbf{84.0}} & 60.0  & 41.1 & 82.9 \\ % Content row 1
\midrule
LDAM & 84.0 & 70.0  & 42.0 & 82.3 \\ % Content row 1
+ALM  & 80.0 & 59.0  & 40.0 & 83.2\\ % Content row 1
+RankReg  & \underline{\textbf{70.3}} & \underline{\textbf{51.6}}  & \underline{\textbf{35.0}} & \textbf{\cl{red!60!white}{84.7}} \\ % Content row 1
\midrule
\textcolor{green!60!black}{Avg.} $\Delta$ & \textcolor{Green}{8.6} & \textcolor{Green}{8.6} & \textcolor{Green}{4.3} & \textcolor{Green}{1.9} \\
\bottomrule % Bottom horizontal line
\end{tabular}
}
\caption{
Comparison results for binary imbalanced CIFAR-100. Baseline numbers are quoted from ALM~\cite{alm}.
} 
\label{tab:cifar100_imb100} 
\end{table}


\begin{table}[t]
\small
\centering % Centres the table on the page, comment out to left-justify
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l c c c c c} 
\toprule % Top horizontal line
& \multicolumn{5}{c}{Melanoma, imb. 1:170} \\ % 
\cmidrule(l){2-6} 
Methods & \vtop{\hbox{\strut FPR@ $\downarrow$}\hbox{\strut  98\%TPR}} & \vtop{\hbox{\strut FPR@ $\downarrow$}\hbox{\strut  95\%TPR}} &\vtop{\hbox{\strut FPR@ $\downarrow$}\hbox{\strut  92\%TPR}} &  \vtop{\hbox{\strut FPR@ $\downarrow$}\hbox{\strut  90\%TPR}} & AUC $\uparrow$ \\ % Column names row
\midrule % In-table horizontal line
BCE & 49.8 & 45.9 & 38.6 & 35.5 & 85.7 \\ % Content row 1
+ALM  & 49.9 & 41.8 & 40.0 & 37.7 & 85.6\\ % Content row 1
+RankReg  & \underline{\textbf{49.4}} & \underline{\textbf{37.9}} & \underline{\textbf{33.9}} & \underline{\textbf{31.6}} & \textbf{\cl{red!60!white}{86.8}} \\ % Content row 1
\midrule
S-ML & \underline{\textbf{46.6}} & 42.8 & 38.4 & 37.4 & 85.3 \\ % Content row 1
+ALM  & 51.3 & \underline{\textbf{40.5}} & 39.8 & 36.2 & 83.5\\ % Content row 1
+RankReg  & 54.6 & 42.4 & \underline{\textbf{36.1}} & \underline{\textbf{34.4}} & \textbf{\cl{red!60!white}{86.3}} \\ % Content row 1
\midrule
S-FL & 59.0 & 47.3 & 44.4 & 39.5 & 83.8 \\ % Content row 1
+ALM  & \underline{\textbf{47.8}} & 42.7 & 39.2 & 38.1 & 84.0\\ % Content row 1
+RankReg   & 56.6 & \underline{\textbf{37.8}} & \underline{\textbf{31.2}} & \underline{\textbf{29.8}} & \textbf{\cl{red!60!white}{86.1}} \\ % Content row 1
\midrule
A-ML & \underline{\textbf{47.5}} & 42.9 & 40.4 & 36.6 & 85.4 \\ % Content row 1
+ALM & 51.0 & 41.5 & 37.5 & 37.1 & 83.7 \\ % Content row 1
+RankReg  & 58.3 & \underline{\textbf{40.8}} & \underline{\textbf{36.7}} & \underline{\textbf{33.9}} & \textbf{\cl{red!60!white}{86.2}} \\ % Content row 1
\midrule
A-FL & 55.6 & 45.0 & 42.7 & 41.2 & 84.4 \\ % Content row 1
+ALM & 49.0 & 42.4 & 40.1 & 38.1 & 83.6\\ % Content row 1
+RankReg  & \underline{\textbf{48.0}} & \underline{\textbf{36.2}} & \underline{\textbf{30.7}} & \underline{\textbf{28.8}} & \textbf{\cl{red!60!white}{86.3}} \\ % Content row 1
\midrule
CB-BCE & 67.2 & 59.5 & 35.7 & 33.2 & 82.6 \\ % Content row 1
+ALM  & 60.8 & 59.5 & 46.3 & 45.8 & 81.5\\ % Content row 1
+RankReg  & \textbf{WIP} \\ 
\midrule
W-BCE & 69.0 & 52.0 & 37.0 & 32.1 & 87.4 \\ % Content row 1
+ALM  & 66.0 & 48.0 & \underline{\textbf{31.0}} & 30.7 & 89.3\\ % Content row 1
+RankReg  & \underline{\textbf{56.4}} & \underline{\textbf{41.1}} & 33.0 & \underline{\textbf{30.5}} & \textbf{\cl{red!60!white}{90.9}} \\ % Content row 1
\midrule
LDAM & 59.7 & 48.2 & 46.2 & 39.0 & 83.4 \\ % Content row 1
+ALM  & 62.7 & 47.7 & 43.3 & 40.7 & 81.5\\ % Content row 1
+RankReg  & \textbf{WIP} \\ 
\bottomrule % Bottom horizontal line
\end{tabular}
}
\caption{ Comparison results for Melanoma dataset.
} 
\label{tab:melanoma} 
\end{table}


\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllllcllll@{}}\toprule[1.2pt]
\multicolumn{1}{c}{\multirow{ 2}{*}{FPR@$\beta$TPR}} & \multicolumn{4}{c}{\textbf{CIFAR100}} & \phantom{abc}& \multicolumn{4}{c}{\textbf{Melanoma}} \\
\cmidrule{2-5} \cmidrule{7-10}
    & 98\%   & 95\%  & 92\% & AUC   && 98\%   & 95\%   & 92\% & AUC \\
 \midrule
Dequeue Max 
& 85.2 & 42.4 & 28.7 & 85.5 && 49.4 & 37.9 & 33.9 & 86.8 \\
FIFO 
& 86.8 & 44.2 & 31.2 & 85.2 && 59.2 & 47.6 & 40.5 & 83.1 \\
\bottomrule[1.2pt]
\end{tabular}
}
\caption{Ablation study on buffer update strategy. Swapping out the most confident sample with incoming ones (\ie Dequeue Max) performs better than first-in-first-out.}
\label{tab:bufferType}
\end{table}

\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllllcllll@{}}\toprule[1.2pt]
\multicolumn{1}{c}{\multirow{ 2}{*}{FPR@$\beta$TPR}} & \multicolumn{4}{c}{\textbf{CIFAR10}} & \phantom{abc}& \multicolumn{4}{c}{\textbf{CIFAR100}} \\
\cmidrule{2-5} \cmidrule{7-10}
    & 98\%   & 95\%  & 92\% & AUC   && 98\%   & 95\%   & 90\% & AUC \\
 \midrule
Buffer = 0 
& 58.8 & 43.6 & 30.2 & 90.4 && 93.4 & 48.4 & 37.4 & 83.1 \\
Buffer = 5 
& 53.0 & 42.4 & 28.7 & 92.6 && 86.6 & 57.2 & 39.0 & 82.5 \\
Buffer = 10 
& 48.1 & 26.9 & 26.2 & 94.5 && 85.2 & 50.2 & 28.7 & 84.6 \\
Buffer = 20 
& 47.6 & 26.2 & 22.0 & 93.8 && 85.2 & 50.0 & 29.8 & 84.9 \\
Buffer = 32 
& 47.1 & 26.2 & 20.6 & 94.3 && 83.0 & 42.4 & 31.4 & 85.5 \\
\bottomrule[1.2pt]
\end{tabular}
}
\caption{False positive rate results at high true positive rates for various buffer sizes.}
\label{tab:bufferSize}
\end{table}
